Reconstruction the scalar-torsion gravity version from the frame of exact cosmological solutions

We consider cosmological models based on the scalar-torsion gravity implying non-minimal coupling between torsion and the scalar field with certain relations between model's parameters. Based on observational constraints on the values of the parameters of cosmological perturbations, the type of the coupling was determined. It was noted that any inflationary models constructed on the basis of the proposed approach can be verified by observational constraints.

==> maikbibl.tex <==
%
% maikbibl.tex 29.11.2001
%
\documentclass[
aps,%
12pt,%
final,%
notitlepage,%
oneside,%
onecolumn,%
nobibnotes,%
nofootinbib,%
superscriptaddress,%
noshowpacs,%
centertags]%
{revtex4}
\bibliographystyle{maik}
\begin{document}
\selectlanguage{english}
\section*{maik.bst}
\nocite{*}
\bibliography{maikbibl}
\end{document}

